A Prototype-Based Neural Network for Image Anomaly Detection and Localization

Image anomaly detection and localization perform not only image-level anomaly classification but also locate pixel-level anomaly regions. Recently, it has received much research attention due to its wide application in various fields. This paper proposes ProtoAD, a prototype-based neural network for image anomaly detection and localization. First, the patch features of normal images are extracted by a deep network pre-trained on nature images. Then, the prototypes of the normal patch features are learned by non-parametric clustering. Finally, we construct an image anomaly localization network (ProtoAD) by appending the feature extraction network with $L2$ feature normalization, a $1\times1$ convolutional layer, a channel max-pooling, and a subtraction operation. We use the prototypes as the kernels of the $1\times1$ convolutional layer; therefore, our neural network does not need a training phase and can conduct anomaly detection and localization in an end-to-end manner. Extensive experiments on two challenging industrial anomaly detection datasets, MVTec AD and BTAD, demonstrate that ProtoAD achieves competitive performance compared to the state-of-the-art methods with a higher inference speed. The source code is available at: https://github.com/98chao/ProtoAD.

==> Tables/tab_finch.tex <==
\begin{table*}[ht]
    \centering
    \caption{Anomaly detection and localization performance of ProtoAD with different FINCH partitions. Each tuple shows image-level AUROC, pixel-level AUROC, and average cluster numbers.}
    \label{tab:finch_result}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c c c c c c}
        \hline
        \bf Category \bf & P2 \bf & P3 \bf & P4 \bf & P5 \bf & P6 \bf & Best \bf & Our \\ \hline
Carpet	    & (99.6, 99.2, 35674) 	& (99.5, 99.2, 1816)   &(100.0, 99.2, 56) 	&(100.0, 99.2, 13 )	&(96.5,98.6, 3)	    &(100.0, 99.2, 56)   &(99.5, 99.2, 1816) \\
Grid	    & (96.7, 98.8, 67994) 	& (94.7, 98.5, 16112)  &(93.7, 98.0, 3983) 	&(92.4, 96.8, 1025) &(85.7,94.8, 260) 	&(96.7, 98.8, 67994) &(93.7, 98.0, 3983) \\
Leather	    & (100.0, 99.4, 13702) 	& (100.0, 99.4, 672)   &(100.0, 99.4,99) 	&(100.0, 99.4, 24 )	&(100.0, 99.4, 6)   &(100.0, 99.4, 6)    &(100.0, 99.4, 672) \\
Tile	    & (99.4, 95.4, 18101) 	& (99.2, 95.2, 826)    &(99.1, 95.0, 51) 	&(98.6, 94.6, 10)   &(97.9, 94.0, 3)	&(99.4, 95.4, 18101) &(99.2, 95.2, 826) \\
Wood	    & (98.9, 95.7, 105187) 	& (99.0, 95.6, 19585)  &(99.1, 95.6, 1639) 	&(99.4, 95.5, 98)   &(98.8, 95.2, 9)	&(99.1, 95.6, 1639)  &(99.1, 95.6, 1639) \\ \hline
\textbf{Texture}& (98.9, 97.7, 48132)& (98.5, 97.6, 7802)  &(98.4, 97.4, 1166) 	&(98.1, 97.1, 234)	&(95.8, 96.4, 56) 	&(99.0, 97.7, 17559) &(98.3, 97.5, 1787) \\ \hline
Bottle	    & (99.9, 98.4, 61108) 	& (99.8, 98.4, 11946)  &(99.9, 98.3, 2106) 	&(99.8, 98.3, 595)	&(99.6, 98.0, 189) 	&(99.9, 98.4, 61108) &(99.9, 98.3, 2106) \\
Cable	    & (99.5, 97.5, 96829) 	& (98.8, 97.7, 21466)  &(98.3, 97.5, 2611) 	&(96.2, 97.0, 535)	&(94.8, 96.3, 136) 	&(99.5, 97.5, 96829) &(98.3, 97.5, 2611) \\
Capsule	    & (94.8, 98.3, 79466) 	& (94.2, 98.3, 12666)  &(93.1, 98.2, 2517) 	&(87.6, 98.0, 2517) &(84.5, 97.6, 235) 	&(94.8, 98.3, 79466) &(93.1, 98.2, 2517) \\
Hazelnut	& (100.0, 98.8, 173989) & (100.0, 98.8, 46894) &(100.0, 98.8, 7127) &(100.0, 98.8, 805) &(99.4, 98.6, 171) 	&(100.0, 98.8, 805)  &(100.0, 98.8, 7127) \\
Metal Nut	& (100.0, 96.7, 91055) 	& (100.0, 96.9, 23558) &(99.9, 96.8, 4969) 	&(99.8, 96.6, 1204) &(99.3, 95.7, 310) 	&(100.0, 96.9, 23558)&(99.9, 96.8, 4969) \\
Pill	    & (96.8, 94.4, 96509) 	& (96.7, 94.6, 17891)  &(95.8, 94.2, 2202) 	&(91.8, 94.0, 519)	&(90.8, 94.5, 147) 	&(96.7, 94.6, 17891) &(95.8, 94.2, 2202) \\
Screw	    & (97.6, 99.0, 129710) 	& (95.5, 99.1, 33990)  &(94.9, 98.9, 5504) 	&(89.4, 98.3, 1140) &(78.8, 97.1, 258) 	&(97.6, 99.0, 129710)&(94.9, 98.9, 5504) \\
Toothbrush	& (100.0, 98.8, 24794) 	& (99.7, 98.8, 5704)   &(99.4, 98.8, 1478) 	&(98.3, 98.7, 417)	&(97.8, 98.4, 108) 	&(100.0, 98.8, 24794)&(99.7, 98.8, 5704) \\
Transistor	& (98.1, 92.9, 104018) 	& (98.3, 93.3, 22724)  &(97.7, 92.5, 4195) 	&(96.6, 90.6, 999)	&(93.5, 87.1, 271) 	&(98.3, 93.3, 22724) &(97.7, 92.5, 4195) \\
Zipper	    & (95.6, 96.7, 71559) 	& (94.6, 96.7, 9323)   &(94.7, 96.6, 1260) 	&(92.5, 96.2, 288)	&(83.7, 95.6, 79)	&(95.6, 96.7, 71559) &(94.6, 96.7, 9323) \\ \hline
\textbf{Object}& (98.2, 97.2, 92904)& (97.8, 97.3, 20616)  &(97.4, 97.1, 3397) 	&(95.2, 96.6, 902)	&(92.2, 95.9, 190) 	&(98.2, 97.2, 52844) &(97.4, 97.1, 4626) \\ \hline
\textbf{All}& (98.5, 97.3, 77980) 	& (98.0, 97.4, 16345)  &(97.7, 97.2, 2653) 	&(96.1, 96.8, 679)	&(93.4, 96.1, 146) 	&(98.5, 97.4, 41083) &(97.7, 97.2, 3680)\\ \hline
    \end{tabular}}
\end{table*}
